DPOK: Reinforcement Learning for Fine-tuning Text-to-Image Diffusion Models

Learning from human feedback has been shown to improve text-to-image models. These techniques first learn a reward function that captures what humans care about in the task and then improve the models based on the learned reward function. Even though relatively simple approaches (e.g., rejection sampling based on reward scores) have been investigated, fine-tuning text-to-image models with the reward function remains challenging. In this work, we propose using online reinforcement learning (RL) to fine-tune text-to-image models. We focus on diffusion models, defining the fine-tuning task as an RL problem, and updating the pre-trained text-to-image diffusion models using policy gradient to maximize the feedback-trained reward. Our approach, coined DPOK, integrates policy optimization with KL regularization. We conduct an analysis of KL regularization for both RL fine-tuning and supervised fine-tuning. In our experiments, we show that DPOK is generally superior to supervised fine-tuning with respect to both image-text alignment and image quality. Our code is available at https://github.com/google-research/google-research/tree/master/dpok.

==> sections/discussion.tex <==
\section{Discussions} \label{sec:disscussion}

In this work, we propose a framework to fine-tune a text-to-image diffusion model as an online RL problem. We show that online RL fine-tuning outperforms simple supervised fine-tuning in improving the model's performance. Also, we conduct an analysis of KL regularization for both methods and discuss the key differences between RL fine-tuning and supervised fine-tuning. 
We believe our work has very clear findings that demonstrate the potential of {\em reinforcement learning from human feedback} in improving text-to-image diffusion models.

%We believe that our work serves as a foundation for the application of {\em reinforcement learning from human feedback} to text-to-image synthesis.
% -- maybe just diffusion models?

% explore online RL fine-tuning for text-to-image diffusion models with KL regularization, and compare it to supervised fine-tuning with KL regularization. 

% We discuss the key differences between both approaches and demonstrate the corresponding empirical results which are aligned with our discussion. Empirical evidence demonstrates that RL fine-tuning consistently outperforms supervised fine-tuning in terms of both image-text alignment and image quality.

% In this work, we explore online RL fine-tuning for text-to-image diffusion models with KL regularization, and compare it to supervised fine-tuning with KL regularization. 
% We discuss the key differences between both approaches and demonstrate the corresponding empirical results which is aligned with our discussion. Empirical evidence demonstrates that RL fine-tuning consistently outperforms supervised fine-tuning in terms of both image-text alignment and image quality.

% To accelerate RL training, one potential approach is to initialize the RL model with the supervised fine-tuned parameters

% {\bf Limitations, future directions}. 
\vspace{-0.05in}
\paragraph{Limitations, future directions.} Several limitations of our work suggest interesting future directions: (a) As discussed in Section~\ref{sec:main_exp}, fine-tuning on multiple prompts requires longer training time, hyper-parameter tuning, and engineering efforts. More efficient training 
% Scaling up to large-scale training 
with a broader range of diverse and complex prompts would be an interesting future direction to explore. (b) Exploring advanced policy gradient methods 
% (e.g., proximal policy optimization~\cite{ppo}) 
can be useful for further performance improvement. Investigating the applicability and benefits of these methods could lead to improvements in the fine-tuning process.

% {\em (b) investigating advanced policy gradient methods.} Even though we utilize a simple vanilla policy gradient for optimization, 


% Stable RL fine-tuning usually requires small learning rates, thus a longer training time is needed compared to supervised fine-tuning. To accelerate RL training, one potential approach is to initialize RL training with the supervised fine-tuned model as in \cite{ouyang2022training}, which could be more beneficial in the multi-prompt training setting.
% %  


% discussion on training with asethetic score

% \section{Conclusion}
% In this work, we explore online RL fine-tuning for text-to-image diffusion models with KL regularization, and compare it to supervised fine-tuning with KL regularization. We discuss the key differences between both approaches and demonstrate the corresponding empirical results which is aligned with our discussion. Empirical evidence demonstrates that RL fine-tuning consistently outperforms supervised fine-tuning in terms of both image-text alignment and image quality.

==> sections/experiments.tex <==
\section{Experimental Evaluation} \label{sec:exp}

% \yd{Note: can move these hypotheses around / edit if needed, but I think it would be nice to initially state \textit{precisely} why we think RL might be better, and how our experiments are designed to ablate each of these different components. I know we have some intuition discussed above about SFT vs RL, but would be good to show that our experiments show this as well!
% We hypothesize that the RL online fine-tuning method leads to better results with respect to both alignment and fidelity for the following reasons:
% \begin{enumerate}
%     \item Hypothesis 1 - RL is better at regularizing towards the initial (prior) data distribution. ((Test this by comparing RL w KL regularization to FT with the same level of KL regularization. Also show that including a large amount of original-dataset data (90\%) in FT training doesn’t fix this.))
%     \item Hypothesis 2 - RL gets more data, whereas SFT overfits to a fixed dataset. ((Test this by training for 1 epoch on an FT dataset which is the same size as the number of samples RL sees.))
%     \item Hypothesis 3 - getting online data is important (for the same reasons online RL in robotics > offline RL). ((Test this by running the FT script iteratively - i.e. generate a small dataset, run FT for an epoch on it, then repeat. If this works well, then it shows online collection matters.))
%     \item Hypothesis 4 - some specific detail of the RL finetuning algorithm matters. ((Test this by ablating details (such as having a baseline) Also maybe compare shortcut fine-tuning with a more standard policy gradient approach which just backdrops through the sampling process?))
% \end{enumerate}
% In the Section X, we present our experimental setup, in Section Y we present our investigations into the hypotheses above, and finally we demonstrate that our method works at scale ... 
% }

We now describe a set of experiments designed to test the efficacy of different fine-tuning baselines and our online RL approach.
% method and report our findings and results.

\subsection{Experimental Setup}

As our baseline generative model, 
we use Stable Diffusion v1.5~\cite{stablediffusion}, which has been pre-trained on large image-text datasets~\cite{laion400m,laion-5b}. For compute-efficient fine-tuning, we use Low-Rank Adaption (LoRA)~\cite{lora}, which freezes the parameters of pre-trained model and introduces low-rank trainable weights. 
%\ow{Maybe mention this in more depth in the related work or method.}
We apply LoRA to the UNet~\cite{unet} module and only update the added weights.
%adds new weights and only updates them. We apply LoRA to Unet and freeze other parameters. 
For the reward model, we use ImageReward~\cite{imagereward} which is trained on a large dataset comprised of human assessments of images. 
Compared to other scoring functions such as CLIP~\cite{clip} or BLIP~\cite{blip}, ImageReward has a better correlation with human judgments, making it the preferred choice for fine-tuning our baseline diffusion model (see Appendix~\ref{app:imagereward} for further justification). Further experimental details (e.g., model architectures, final hyper-parameters) are provided in Appendix~\ref{app:exp}.


% \begin{figure} [t] \centering
% \includegraphics[width=.9\textwidth]{figures/single_prompt_seen_v2.pdf}
% \caption{Samples from the Stable Diffusion version 1.5 (SD 1.5), supervised fine-tuning (SFT) model, RL fine-tuning model and Stable Diffusion version 2.0 (SD 2.0).}
% \label{fig:seen_fig}
% \end{figure}


\begin{figure*} [t!] \centering
\subfigure[Seen text prompt]
{
\includegraphics[width=0.9\textwidth]{figures/single_prompt_seen_v5.pdf}
\label{fig:main_fig_0}} 
\subfigure[Unseen text prompt]
{\includegraphics[width=0.9\textwidth]{figures/single_prompt_unseen_v5.pdf}
\label{fig:main_fig_2}}
\caption{Comparison of images generated by the original Stable Diffusion model, supervised fine-tuned (SFT) model, and RL fine-tuned model. Images in the same column are generated with the same random seed. (a) Images from seen text prompt: ``A green colored rabbit'' (color), ``A cat and a dog'' (composition), ``Four wolves in the park'' (count), and ``A dog on the moon'' (location). (b) Images from unseen text prompt: ``A green colored cat'' (color), ``A cat and a cup'' (composition), ``Four birds in the park'' (count), and ``A lion on the moon'' (location).} 
%\ow{If the images were randomly sampled mention this so it's clear they aren't cherrypicked.}}
\label{fig:main_fig}
\end{figure*}


\begin{figure*} [t!] \centering
\subfigure[ImageReward]
{
\includegraphics[width=0.48\textwidth]{figures/reward_train.pdf}
\label{fig:reward_seen}} 
\subfigure[Aesthetic score]
{\includegraphics[width=0.48\textwidth]{figures/aesthetic_train.pdf}
\label{fig:reward_unseen}}
\caption{(a) ImageReward scores and (b) Aesthetic scores of three models: the original model, supervised fine-tuned (SFT) model, and RL fine-tuned model. ImageReward and Aesthetic scores are averaged over 50 samples from each model.}
\label{fig:reward_main}
\end{figure*}

\subsection{Comparison of Supervised and RL Fine-tuning} \label{sec:main_exp}

%\paragraph{Single prompt training.}
We first evaluate the performance of the original and fine-tuned text-to-image models w.r.t.\ specific capabilities, such as generating objects with specific colors, counts, or locations;  and composing multiple objects (or \emph{composition}). For both RL and SFT training we include KL regularization (see hyperparameters in Appendix~\ref{app:exp}).
To systematically analyze the effects of different fine-tuning methods, we adopt a straightforward setup that uses one text prompt during fine-tuning.
As training text prompts, we use ``A green colored rabbit'', ``A cat and a dog'', ``Four wolves in the park'', and ``A dog on the moon''. These test the models' ability to handle prompts involving {\em color}, {\em composition}, {\em counting} and {\em location}, respectively.
For supervised fine-tuning, we use 20K images generated by the original model, which is the same number of (online) images used by RL fine-tuning.
% for a fair comparison. 

% \textcolor{red}{(we should also mention KL regularization settings here, maybe refer to appendix)}

% To systematically analyze the effects of different fine-tuning methods,
% we consider a straightforward setup that involves one text prompt during fine-tuning.
% We generate a text prompt by combining a descriptive word or phrase with some object (e.g., combining {\em Four} with {\em wolves}).
% We evaluate the performance of a text-to-image model's specific abilities, such as composing multiple objects ({\em composition}) and generating  objects with specific colors, counts, and locations.
% generating an object 
% we consider four categories: {\em color}, {\em composition}, {\em counting} and {\em location}. 
% To create text prompts for each category, we combine a descriptive word or phrase with some object (e.g., combining {\em Four} with {\em wolves}). 
% For supervised fine-tuning, we use 20K images generated by the original model, which matches the total number of images used for RL fine-tuning.

%are utilized.\footnote{We maintain a consistent total number of images for both supervised fine-tuning and RL fine-tuning to investigate the importance of online learning.}

%which the original model struggles to handle correctly (see Figure~\ref{fig:main_fig_0}).
%For supervised fine-tuning, we generate 10K images using the original model and select 1K images that have an ImageReward score of 1 or greater. 
%(\textcolor{red}{the same number of samples})
%For fair comparison, we maintain a consistent total number of optimization steps for both supervised fine-tuning and RL fine-tuning. (Ying:\textcolor{red}{Why the same optimization steps? they don't even use the same learning rate and the same algorithm? How about training to convergence?})

Figure~\ref{fig:reward_seen} compares ImageReward scores of images generated by the different models (with the same random seed). 
%\ow{It seems odd to use ImageReward scores as the main alignment metric since both finetuning methods directly optimize against it. At least we should point this out as a potential limitation of the metric.} 
We see that both supervised fine-tuning (SFT) and RL fine-tuning improve the ImageReward scores on the training text prompt.
This implies the fine-tuned models can generate images that are better aligned with the input text prompts because ImageReward is trained on human feedback datasets to evaluate image-text alignment.
%\textcolor{red}{[kiminl]: depending on new runs on SFT, we can argue that RL is better than SFT in maximizing rewards.}
% Figure~\ref{fig:reward_seen} shows the images generated by the original model and fine-tuned models with the same random seed.
% One can recognize that the image-text alignment is improved after fine-tuning.
%, fine-tuned models indeed show a better image-text alignment compared to the original model. 
Figure~\ref{fig:main_fig_0} indeed shows that 
% with the same random seed,
fine-tuned models add objects to match the number (e.g., adding more wolves in ``Four wolves in the park''), and replace incorrect objects with target objects (e.g., replacing an astronaut with a dog in ``A dog on the moon'') compared to images from the original model.
%generate missing objects (adding wolves to match the number in ``Four wolves in the park'' or replacing an astronaut with a dog in ``A dog on the moon'') to match the input text prompts. 
They also avoid obvious mistakes like generating a rabbit with a green background given the prompt ``A green colored rabbit''. Of special note, fine-tuned models generate better images than the original model on several unseen text prompts consisting of unseen objects in terms of image-text alignment (see Figure~\ref{fig:main_fig_2}).
% \cb{Why is there no discussion of RL vs.\ SFT w.r.t.\ ImageReward?} 

As we can observe in Figure~\ref{fig:reward_seen}, RL models enjoy higher ImageReward then SFT models when evaluated with the same training prompt in different categories respectively, due to the benefit of online training as we discuss in Section~\ref{sec:contrast}.
We also evaluate the image quality of the three models using the aesthetic predictor~\cite{laion-5b}, which is trained to predict the aesthetic aspects of generated images.\footnote{The aesthetic predictor had been utilized to filter out the low-quality images in training data for Stable Diffusion models.} 
%\ow{explain what this is}; see Figure~\ref{fig:reward_unseen}.
Figure~\ref{fig:reward_unseen} shows that supervised fine-tuning degrades image quality relative to the RL approach (and sometimes relative to the pre-trained model), even with KL regularization which is intended to blunt such effects.
%While both fine-tuning approaches offer strong text-image alignment, we see that supervised fine-tuning degrades image quality relative to the RL approach (and sometimes relative to the pretrained model), even with KL regularization which is intended to blunt such effects. 
For example, the supervised model often generates over-saturated images, corroborating the observations of \citet{lee2023aligning}. By contrast, the RL model generates more natural images that are at least as well-aligned with text prompts. 

% The aesthetic score of RL model is improved while SFT model has lower scores.
%aesthetic score~\cite{laion-5b}, which is trained for image quality evaluation. Figure~\cite{fig:reward_unseen} shows that the 
%\textcolor{red}{[to-do] add hypothesis to explain why}

Even though we mainly focus on the straightforward setup with a single training text prompt for systemic analysis,
we remark that fine-tuning on multiple prompts can also improve the pre-trained model across multiple categories, and also work with long and complex prompts (see Appendix~\ref{app:multiprompt} for supporting results).
However, we also observe that longer training time, hyper-parameter tuning, and engineering efforts are required as the number of training text prompts increase, and we defer further investigation of fine-tuning on multiple prompts to future work.
%\footnote{One can interpret fine-tuning on multi prompts as multi-task RL where each text prompt corresponds to one environment. Usually, multi-task RL requires advanced techniques for stable training.}

% To systematically analyze the effects of different fine-tuning methods, we adopt a straightforward setup 
% \textcolor{red}{We remark that fine-tuning on multiple prompts is also working well. However, training on multi-prompts requires more training and engineering. original=0.47, rl=1.11, sup=0.98 on multi1}
% See results in Appendix~\ref{app:multiprompt}.


\subsection{The Effect of KL Regularization: Online RL versus Supervised Fine-tuning} \label{sec:kl_abl}

% \begin{figure} [h] \centering
% \includegraphics[width=.75\textwidth]{figures/ablation_kl.pdf}
% \caption{Comparison of images generated by RL models and SFT models optimized with and without KL regularization. We use ``A green colored rabbit.'' as training text prompt. Images in the same column are generated with the same random seed.}
% % . To verify the effects of KL regularization, 
% % f
% % using RL and SFT fine-tuning, with and without KL regularization, fine-tuned on the single prompt ``A green colored rabbit.''}
% \label{fig:kl}
% \end{figure}

\begin{figure*} [t] \centering
\vspace{-0.1in}
\subfigure[ImageReward and Aesthetic scores]
{
\includegraphics[width=0.46\textwidth]{figures/reward_kl_new.pdf}
\label{fig:im_kl}} 
\subfigure[Generated images]
{\includegraphics[width=0.5\textwidth]{figures/ablation_kl.pdf}
\label{fig:img_kl}}
\vspace{-0.1in}
\caption{Ablation study of KL regularization in both SFT and RL training, trained on single prompt ``A green colored rabbit''. (a) 
ImageReward and Aesthetic scores are averaged over 50 samples from each model. (b) Images generated by RL models and SFT models optimized with and without KL regularization. Images in the same column are generated with the same random seed.}
\vspace{-0.1in}
\label{fig:im_as_kl}
\end{figure*}
% what to put here?
% \paragraph{Control the number of samples in both SFT and RL training}

To demonstrate the impact of KL regularization on both supervised fine-tuning (SFT) and online RL fine-tuning, 
we conduct an ablation study, fine-tuning the pre-trained model with and without KL regularization on ``A green colored rabbit''.
Figure~\ref{fig:im_kl} shows that KL regularization in online RL is effective in attaining both high reward and aesthetic scores.
We observe that RL model without KL regularization generates low-quality  images (e.g., oversaturated colors and unnatural shapes) as shown in Figure~\ref{fig:img_kl}.
In the case of SFT, 
KL regularization reduces the ImageReward score while slightly improving the aesthetic score.
However, one can note that the visual quality of generated samples is similar (see Figure~\ref{fig:img_kl}).
% is not very effective in stabilizing the fine-tuning. 
% It slightly improves the aesthetic score but visual quality of generated samples is similar.
%KL regularization is not very effective in stabilizing the fine-tuning. 
%It slightly improves the aesthetic score but visual quality of generated samples is similar.
%while sacrificing ImageReward score.
We expect that this is due to the different nature of online and offline training---KL regularization is only applied to fixed samples in the case of SFT while KL regularization is applied to new samples per each update in the case of online RL (see Section~\ref{sec:contrast} for related discussions).



% We demonstrate the impact of KL regularization on both supervised fine-tuning and online RL fine-tuning, using the single training prompt ``A green colored rabbit.''.
% %as an example.
% We fine-tune models using both RL and SFT approaches with and without KL regularization.
% Online RL-based KL regularization is more effective in attaining both high alignment and high fidelity compared to supervised KL. In the supervised approach, adding supervised KL improves the aesthetic score while sacrificing ImageReward score. By contrast, in online RL training, adding online KL regularization does not generally reduce the reward given the right choice of KL weight, mainly due to the different nature of online and offline training---the online model is free to explore image space more freely.
% % while that enjoys both high reward and low online KL loss. 
% However, for supervised KL regularization, it would increase the reward score equivalently for each sample in the pre-trained dataset regardless of whether it has high or low reward, leading to a decrease in the reward\footnote{One extreme case is $\gamma \geq r$, which would assign almost equivalent weights for all samples during supervised fine-tuning regardless of the reward.}.

% commented out for arxiv version
We also include more results for SFT models with KL regularization in Appendix~\ref{app: sup_kl}, which shows that even with different choices of the KL weight, the KL regularization is not very effective in improving the visual quality.
%SFT with KL still reduces the reward score.


\begin{figure} [ht] \centering
\includegraphics[width=.99\textwidth]{figures/ablation_four_rouses.pdf}
\caption{Comparison of images generated by the original model and RL fine-tuned model on text prompt ``Four roses''. The original model, which is trained on large-scale datasets from the web~\cite{laion-5b,laion400m}, tends to produce whiskey-related images from ``Four roses'' due to the existence of a whiskey brand bearing the same name as the prompt. In contrast, RL fine-tuned model with ImageReward generates images associated with the flower ``rose''.}
\vspace{-0.15in}
\label{fig:four}
\end{figure}





% \textcolor{red}{show the training results on long prompt just to show the improvement on details which cannot be achieved by sft -- gain from rl}
% %both seen and unseen text prompts. However, due to online updates, RL is more effective than supervised fine-tuning in maximizing the scores. 
% Figure~\ref{fig:main_fig} shows image samples from the original model, SFT model and RL model. As observed in \cite{lee2023aligning}, SFT model has several issues like oversaturated colors, while RL model generates high-quality images. We expect that this is because RL fine-tuned model keeps receiving the signals on updated outputs. 

\subsection{Reducing Bias in the Pre-trained Model}

To see the benefits of maximizing ImageReward, we explore the effect of RL fine-tuning in reducing bias in the pre-trained model.  Because the original Stable Diffusion model is trained on large-scale datasets extracted from the web~\cite{laion400m,laion-5b}, it can encode some biases in the training data. As shown in Figure~\ref{fig:four}, we see that the original model tends to produce whiskey-related images given the prompt ``Four roses'' (which happens to be the brand name of a whiskey), which is not aligned with users' intention in general.
%clearly shows some biased behaviors. 
To verify whether maximizing a reward model derived from human feedback can mitigate this issue, we fine-tune the original model on the ``Four roses'' prompt using RL fine-tuning.
Figure~\ref{fig:four} shows that the fine-tuned model generates images with roses (the flower) because the ImageReward score is low on the biased images (ImageReward score is increased to 1.12 from -0.52 after fine-tuning).
This shows the clear benefits of learning from human feedback to better align existing text-to-image models with human intentions.

% However, RL fine-tuned model does not generate

% fine-tuning with ImageReward on “Four roses” can reduce such unintended bias in the original model. Because ImageReward is trained on human datasets, this reward function produces low scores on biased images and thus fine-tuned model
% can generate




% \paragraph{KL regularization.}

%\subsection{Multi-prompt training}

% \begin{figure} [t] \centering
% \includegraphics[width=.9\textwidth]{figures/multi_prompt.pdf}
% \caption{Samples from the original Stable Diffusion model and RL fine-tuned model on multiple text prompts from DrawBench.}
% \label{fig:multi}
% \end{figure}

==> sections/intro.tex <==
\section{Introduction} \label{sec:intro}

% Success of text-to-image models 
Recent advances in \emph{diffusion models}~\cite{ho2020denoising, sohl2015deep,ddim}, together with pre-trained text encoders (e.g., CLIP~\cite{clip}, T5~\cite{t5}) have led to impressive results in text-to-image generation.
Large-scale text-to-image models, such as Imagen~\cite{imagen}, Dalle-2~\cite{dalle2} and Stable Diffusion~\cite{stablediffusion}, generates high-quality, creative images given novel text prompts. However, despite these advances, current models are often lacking in certain. For example, current models have a limited ability to compose multiple objects~\cite{feng2022training,gokhale2022benchmarking,petsiuk2022human}. They also frequently encounter difficulties when generating objects with specified colors and counts~\cite{tifa,lee2023aligning}.

% recent approaches 
\emph{Learning from human feedback (LHF)} has proven to be an effective means to overcome these limitations~\cite{pickscore,lee2023aligning,hps,imagereward}.
\citet{lee2023aligning} demonstrate that certain properties, such as generating objects with specific colors, counts, and backgrounds, can be improved by learning a \emph{reward function} from human feedback, followed by fine-tuning the text-to-image model using supervised learning. 
They show that simple supervised fine-tuning based on reward-weighted loss can improve the reward scores, leading to better image-text alignment.
However, 
supervised fine-tuning often induces a deterioration in image quality (e.g., over-saturated or non-photorealistic images). 
This is likely due to the model being fine-tuned on a fixed dataset that is generated by the pre-trained model (see Figure~\ref{fig:framework_sup}).
%, and potential over-fitting to the reward model with the fixed data. 
% One would imagine that adding some KL regularization would mitigate the issue, but we also tried it. -- discussed later in intro 

% \ow{I'm not very convinced by the argument is limited samples/overfitting since our reward model lets us label arbitrarily large datasets. Do we have an experiment where the dataset is large enough that we only take 1 pass over the dataset to show that overfitting isn't an issue there?  If the image quality issues remain, it seems more likely the issue is distribution shift.
% This claim that small dataset --> overfitting --> poor image quality also seems inconsistent with works like DreamBooth, which use a super small set of images but maintain high quality.
% }
% Despite of simplicity and effectiveness in improving image-text alignment, this supervised learning method also reduces the image quality (e.g., generating oversaturated and non-photorealistic images). One can expect that this is because the model is fine-tuned on a fixed supervised dataset.

%the interest in learning from human feedback has been increased~\cite{lee2023aligning,pickscore,imagereward,hps}.

% \citet{pickscore} and \citet{imagereward} have collected large-scale human feedback datasets and trained reward functions called, PickScore and ImageReward, respectively. 

% PickScore~\cite{pickscore}, ImageReward~\cite{imagereward}, HPS~\cite{hps},TIFA~\cite{tifa}

% our approach
% \textcolor{red}{[ying@: could you summarize our approach?]}


\begin{figure*} [t!] \centering
\subfigure[Supervised fine-tuning]
{
\includegraphics[width=0.45\textwidth]{figures/main_figure_v3.pdf}
\label{fig:framework_sup}} 
\subfigure[RL fine-tuning]
{\includegraphics[width=0.45\textwidth]{figures/main_figure_v2.pdf}
\label{fig:framework_rl}}
\caption{Illustration of (a) supervised fine-tuning and (b) RL fine-tuning. Both start with the same pre-trained model (the blue rectangle). In supervised fine-tuning, the model is updated on a fixed dataset generated by the pre-trained model. In contrast, the model is updated using new samples from the previously trained model during RL fine-tuning.}
\label{fig:framework}
\end{figure*}

% \begin{figure*} [t] \centering
% \includegraphics[width=.95\textwidth]{figures/main_figure.pdf}
% \caption{Illustration. }
% \label{fig:framework}
% \end{figure*}

%To achieve better text-image alignment still maintaining high image fidelity, 
In this work, we explore using \emph{online reinforcement learning (RL)} for fine-tuning text-to-image diffusion models.
%using a reward function that is learned from human feedback. 
We show that optimizing the expected reward of a diffusion model's image output is equivalent to performing policy gradient on a multi-step diffusion model under certain regularity assumptions. We also incorporate Kullback–Leibler (KL) divergence w.r.t.\ the pre-trained model, as regularization in an online manner, treating this as an implicit reward.
%\textcolor{red}{to stabilize RL fine-tuning. -- how about just as regularization?} 

In our experiments, we fine-tune the Stable Diffusion model~\cite{stablediffusion} using ImageReward~\cite{imagereward}, which is trained on a large dataset comprised of human assessments of images.
We show that online RL fine-tuning achieves 
% ceb: don't say expected reward here...
% high expected reward
strong text-image alignment
while maintaining high image fidelity by optimizing its objective in an online manner. \emph{Crucially, online training allows evaluation of the reward model (see Figure~\ref{fig:framework_rl}) and conditional KL divergence beyond the (supervised) training dataset}. This offers distinct advantages over supervised fine-tuning, a point we demonstrate empirically. In our empirical comparisons, we also incorporate the KL regularizer in a supervised fine-tuning method for a fair comparison.

% and compare it with the supervised fine-tuning approach, both with KL regularization w.r.t. the pre-trained model but in different manners. 

% First, we show that optimizing the expected reward of the final image output is equivalent to performing policy gradient on multi-step diffusion models under regularity assumptions. We also explore KL regularization with respect to the pre-trained model in an online manner as an implicit reward for fidelity. Finally, as an fair comparison, we adopt a KL regularization term under the supervised fine-tuning setting, and compare it to the online approach. 
% Empirically, we show that by online fine-tuning, we can achieve both high expected reward while maintaining high fidelity thanks to optimizing the objective in an online manner, which allows evaluation of the reward model and conditional KL divergence outside of the supervised learning dataset; In contrast, for the supervised setting, even if we add the KL regularization term, it is still hard to achieve both high reward and fidelity due to the limitation of imitating some fixed behavior and not able to explore outside of the supervised data. 
% We also discuss the fundamental difference between supervised fine-tuning and online fine-tuning for text-to-image models, where we argue that online fine-tuning can benefit from a good reward model to provide more reward signals compared to supervised fine-tuning with its generalization ability of the reward model to extrapolate outside the supervised training dataset.

 
Our contributions are as follows:

\begin{itemize} [leftmargin=7mm]
    \item We frame the optimization of the expected reward (w.r.t.\ an LHF-reward) of the image output from a diffusion model given text prompts as an online RL problem. 
    % and show that under certain regularity assumptions, optimizing this expected reward is equivalent to policy gradient.

    \item We propose the use of KL regularization w.r.t.\ the pre-trained text-to-image model as an implicit reward to stabilize RL fine-tuning.
    %to encourage image fidelity in our online setting.

    \item We also study incorporating KL regularization into supervised fine-tuning of diffusion models (which allows a fairer comparison with our RL technique).

    % \item We explore different design choices for both online fine-tuning and supervised fine-tuning methods.

    \item We discuss key differences between supervised fine-tuning and online fine-tuning of text-to-image models, arguing that online fine-tuning is critical to improving text-to-image alignment while maintaining high image fidelity.
    % and also show other benefits from online fine-tuning such as generalization abilities.
\end{itemize}

% experimental results




==> sections/method.tex <==
\section{Online RL Fine-tuning of Diffusion Models}
\label{sec:main}

% \ow{General comment: I suggest starting with the motivation for each of the algorithms below (e.g. explain the intuition for treating the diffusion process as a sequence, then show the algo for it; explain the need for regularization, then show the algo).}

In this section, we detail our approach for online RL fine-tuning of diffusion models. 
Our approach incorporates a KL term to ensure that the updated model is not too far from the original model.
%, with a KL term incorporated in order to maintain image fidelity while improving alignment.
For comparison, we also present a modified supervised fine-tuning method with KL regularization, and discuss the difference between these two approaches.


% In this section, we discuss online fine-tuning and supervised fine-tuning, both with KL regularization to maintain high fidelity while improving alignment, and discuss the difference between these two approaches.

% \yd{Rewriting a bit for clarity (feel free to use/ignore as you see fit!): In this section, we detail our proposed approach for online RL fine-tuning of diffusion models, with a KL term incorporated for maintaining high fidelty while improving alignment. As an ablation, we also present a supervised fine-tuning method with KL regularization, and discuss the difference between these two approaches.}


\subsection{RL Fine-tuning with KL Regularization}

% ceb: I suggest removing these para headings. They add nothing and brea up the flow.
% \paragraph{Online training objective.}
We first outline the primary approach.
Let $p_\theta(x_{0:T}|z)$ be a text-to-image diffusion model where $z$ is some text prompt distributed according to $p(z)$, and let $r(x_0,z)$ be a reward model (typically trained using human assessment of images). Our goal is to re-train/fine-tune the diffusion model to maximize the expected reward of the generated images given the prompt distribution, i.e.,% minimizing the objective below:
%Given a text-to-image diffusion model $p_\theta(x_{0:T}|z)$ where $z$ is some text prompt, we consider maximizing the expected reward over a distribution of prompts $p(z)$:
%
\begin{align}
\label{eq:online-objective}
\min_\theta \; \mathbb{E}_{p(z)}\mathbb{E}_{p_\theta(x_0|z)}[- r(x_0,z)].
\end{align}
We obtain the following gradient of this objective function:
\begin{lemma}[A modification of Theorem 4.1 in \cite{fan2023optimizing}]
\label{lemma_pg}
If $p_\theta(x_{0:T}|z)r(x_0,z)$ and $\nabla_{\theta}p_\theta(x_{0:T}|z)r(x_0,z)$ are continuous functions of $\theta$, $x_{0:T}$, and $z$, then we can write the gradient of the objective in~\eqref{eq:online-objective} as 
%
\begin{equation}
  \label{eq:pg}
  \nabla_{\theta} \mathbb{E}_{p(z)}\mathbb{E}_{p_\theta(x_0|z)}[-r(x_0,z)] = \mathbb{E}_{p(z)}\mathbb{E}_{p_\theta(x_{0:T}|z)}\left[-r(x_0,z) \sum_{t=1}^{T} \nabla_{\theta}\log p_{\theta}(x_{t-1}|x_{t},z)  \right] . 
\end{equation}
%   
\end{lemma}

\begin{proof}
    We present the proof in Appendix~\ref{proof_pg}.
\end{proof}

% \paragraph{MDP construction.}

We can construct a Markov decision process (MDP), with a finite horizon $T$, that captures the dynamics of the diffusion model. Specifically, we treat  $p_{\theta}(x_{t-1}|x_{t},z)$ as a \emph{policy} given prompt $z$. Given $x_t$. the action is $a = x_{t-1}$, and the next state given by the "environment" is identical to the action. The reward is
$r(x_0,z)$ at the final step, and $0$ at any other step. On this view, Eq.~(\ref{eq:pg}) is equivalent to performing policy gradient in the MDP. {Note that we keep the covariance $\Sigma_t$ as constant in DDPM and only train $\mu_\theta$, such that it would naturally provide a stochastic policy for online exploration. 

}

% \paragraph{Discussion.} 

Notice that this RL-based policy gradient approach is not the only way to optimize objective~(\ref{eq:pg}). Alternatively, one could compute the gradient through the trajectories to update the model; but the multi-step nature of diffusion models makes this approach memory inefficient and potentially prone to numerical instability. Consequently, scaling it to high-resolution images becomes challenging.
%means this is highly memory inefficient and may induce numerical instability. This, in turns, makes it difficult to scale to high-resolution images.
% \ow{Why is this hard? Memory issues? If so, group those phrases together.} 
For this reason, we adopt policy gradient to train large-scale diffusion models like Stable Diffusion~\cite{stablediffusion}.
% discussion: why policy gradient? direct optimization is highly memory expensive

% \ow{I'd recommend moving this paragraph to the start of section 4.1 to motivate why we're doing this.}


% discussion: 


\paragraph{KL regularization in an online manner.} 

% Note that the reward model is generally trained to reflect the alignment between image and text, which might not necessarily reflect the image quality. 

% \ow{Following prior work [cite a few examples...]} 
The risk of fine-tuning based purely on the LHF-generated reward model is that may discount the ``skill'' of the initial diffusion model to a greater degree than warranted. To avoid over-fitting the reward model, we incorporate the KL divergence between the fine-tuned model and the pre-trained model as a regularizer.
We consider KL divergence between the current model and the pre-trained model as a regularization term 
%to avoid over-fitting to the reward model, 
similar to~\cite{ouyang2022training,stiennon2020learning}. 
% \textcolor{red}{@ying: could you add some motivations about KL regularization here?}
% We first observe:
\begin{lemma}
\label{lemma_online_kl} Assume that $p_\text{pre}(x_{0:T}|z)$ and $p_\theta(x_{0:T}|z)$ are both Markov chains starting from $x_T\sim\mathcal{N}(0,I)$ given text prompt $z$. Then we have
%
\begin{align}
\mathbb{E}_{p(z)}\! [\text{\em KL}(p_\theta (x_0 | z)) \| p_{\text{pre}}(x_0 | z))] \!\leq \! \mathbb{E}_{p(z)}\! \left[\sum_{t=1}^{T}\! \mathbb{E}_{p_\theta(x_{t}|z)}\! \big[\! \text{\em KL}\big(p_\theta(x_{t-1} | x_t,z) \| p_{\text{pre}}(x_{t-1} | x_t, z)\! \big)\! \big]\!\right] \!.
% \mathbb{E}_{p(z)}\big[\text{\em KL}\big(p_\theta(x_0|z) \| p_{\text{pre}}(x_0|z)\big)\big] &\leq \mathbb{E}_{p(z)}\mathbb{E}_{p_\theta(x_{0:T}|z)}\left[\sum_{t=1}^{T}\log \frac{p_\theta(x_{t-1}|x_t,z)}{p_{\text{pre}}(x_{t-1}|x_t,z)}\right] \\
% &= \mathbb{E}_{p(z)}\Big[\sum_{t=1}^T\mathbb{E}_{p_\theta(x_t|z)}\big[\text{\em KL}\big(p_\theta(x_{t-1}|x_t,z) \| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big]\Big]. \nonumber 
\end{align}
%
\end{lemma}
See derivation in Appendix~\ref{app: online_kl}.
Empirically, we use a combined objective function:
% Using the lemma above, for online fine-tuning, we  regularize $\sum_{t=1}^T\mathbb{E}_{p_\theta(x_t)}\big[\text{KL}\big(p_\theta(x_{t-1}|x_t,z)\| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big]$ at each step $t\leq T$.
% % given any $z$. Note that from 
% By the product rule, we have
% %
% \begin{align}
% \label{partial_grad}
% &\sum_{t=1}^T\nabla_\theta\mathbb{E}_{p_\theta(x_t)}\big[\text{KL}\big(p_\theta(x_{t-1}|x_t,z) \| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big] \nonumber \\
% &\quad= \sum_{t=1}^T\mathbb{E}_{p_\theta(x_t)}\big[\nabla_\theta \text{KL}\big(p_\theta(x_{t-1}|x_t,z) \| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big] \\ 
% &\quad+\sum_{t=1}^T\mathbb{E}_{p_\theta(x_t)}\big[\nabla_\theta \log p_\theta(x_t)\cdot\text{KL}\big(p_\theta(x_{t-1}|x_t,z) \| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big]. \nonumber
% \end{align}
% % 
% Moreover, the second term in Eq.~(\ref{partial_grad}) can be rewritten as
% %
% \begin{equation}
% \begin{aligned}
% &\sum_{t=1}^T\mathbb{E}_{p_\theta(x_t)}\big[\nabla_\theta \log p_\theta(x_t) \cdot \text{KL}\big(p_\theta(x_{t-1}|x_t,z) \| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big] \\
% & \quad= \sum_{t=1}^T\mathbb{E}_{p_\theta(x_t)}\big[\sum_{t'>t}^T \nabla_\theta \log p_\theta(x_{t'-1}|x_{t'}, z) \cdot \text{KL}\big(p_\theta(x_{t-1}|x_t,z) \| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big], 
% \end{aligned}   
% \end{equation}
% %
% which treats the sum of conditional KL-divergences along the prior sub-trajectory as a scalar reward at each step. However, computing these sums is more inefficient than just the first term in Eq.~(\ref{partial_grad}). Empirically, we find that regularizing only the first term in Eq.~(\ref{partial_grad}) works well, 
% % so we adopt the first term in Eq.~(\ref{partial_grad}) when calculating the gradient for simplicity, 
% so we adopt this approach for simplicity, which yields the KL-regularized objective: 

% (another lemma)

% Since distribution of $x_0$ is generally not tractable, we consider an upper bound in the lemma below.

% \begin{lemma}
% \label{lemma_online_kl}
% If both $p_\theta$ and $p_{\text{pre}}$ are Markov chains starting from the same distribution $x_T \sim \mathcal{N}(0, I)$ given any $z$, then
% \begin{equation}
% \mathbb{E}_{p(z)}[\text{KL}(p_\theta(x_0|z)\| p_{\text{pre}}(x_0|z))] \leq\mathbb{E}_{p(z)}\mathbb{E}_{p_\theta(x_{0:T}|z)}\left[\sum_{t=1}^{T}\log \frac{p_\theta(x_{t-1}|x_t,z)}{p_{\text{pre}}(x_{t-1}|x_t,z)}\right]
% \end{equation}
% \end{lemma}

% Derivation is in Appendix~\ref{proof_online_kl}.
% See proof in Appendix~\ref{}. 
% discussion: difference between sft and online ft

% \paragraph{Importance sampling.}
% \paragraph{Objective function for online fine-tuning with KL regularization.}

\begin{equation}
\label{eq:online}
\begin{aligned}
&\mathbb{E}_{p(z)}\left[\alpha\mathbb{E}_{p_\theta^*(x_{0:T}|z)}[- r(x_0,z) \sum_{t=1}^{T} \log p_{\theta}(x_{t-1}|x_{t},z)  ] \right.\\
&\left . + \beta\sum_{t=1}^{T}\mathbb{E}_{p_\theta^*(x_{t}|z)}\big[\text{KL}\big(p_\theta(x_{t-1}|x_t,z) \| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big]\right] .   
\end{aligned}
\end{equation}
Here $\alpha, \beta$ are the reward weight and KL weight, respectively, and we use the notation $p_\theta^*$ to indicate that we treat it as constant when calculating the gradient. To see the difference between the upper bound in Lemma~\ref{lemma_online_kl} and the KL regularization term in eq.~(\ref{eq:online}),  and why we use the latter one for experiments, please refer to Appendix~\ref{app: partial_gradient}. 

We present the algorithm for RL fine-tuning in Algorithm~\ref{algo: RL}. 
% \red{In practice, sampling new images is one of the speed bottleneck in training \ow{True?}. To perform more gradient steps without resampling, we perform multiple gradient steps per sampling step and use importance sampling to handle off-policy samples.}
%\textcolor{red}{[kimin]: expectation in eq(7) looks like we need to sample entire trajectory as one data point but we are actually smapling one transition. Is this ok? I may miss something. -- we can view that as we sample from the distribution of $x_{0:T}$} 

\begin{algorithm}[t]
  \caption{RL fine-tuning for diffusion models with human feedback}

% \textbf{Require:} 
\textbf{Input}: Reward model $r$, pre-trained diffusion model $p_\text{pre}$, diffusion model $p_\theta$, sampling batch size $m$, training batch size $n$, reward weight $\alpha$, KL weight $\beta$, text distribution $p(z)$

\begin{algorithmic}
\STATE Initialize $p_\theta = p_\text{pre}$
\WHILE{$\theta$ not converged}
%  \FOR{t = 0,...,$n_{\text{critic}}$}
\STATE Obtain $m$ i.i.d. samples by first sampling $z\sim p(z)$ and then ${x_{0:T}} \sim p_{\theta}({x_{0:T}}|z)$

\STATE Randomly select $n$ transition samples, final output and text condition: $\{x_{t-1}, x_{t}, x_0, z\}$

\STATE Take gradient step on $$\nabla_\theta \big(-\alpha r(x_0,z)\log p_\theta(x_{t-1}|x_t,z) + \beta \text{KL}\big(p_\theta(x_{t-1}|x_t,z) \| p_{\text{pre}}(x_{t-1}|x_t, z)\big)\big)$$
% \STATE Obtain $m$ i.i.d. samples from $q_0$ 
% \STATE Update $\alpha$ and $\omega$ via maximizing Eq.~(\ref{eq: b and c})
% \ENDFOR
\ENDWHILE
\end{algorithmic}
\label{algo: RL}
\textbf{Output}: Fine-tuned diffusion model $p_\theta$
\end{algorithm}

\subsection{Supervised Learning with KL Regularization}

% ceb: This section does not discuss the differences (??)
% In this section, we introduce the objective functions for supervised fine-tuning also compare the differences between supervised fine-tuning and online fine-tuning with KL regularization.

We now introduce KL regularization into supervised fine-tuning (which allows a more meaningful comparison with our KL-regularized RL technique).
%
% \paragraph{Supervised fine-tuning objective.}
%
We begin with a supervised fine-tuning objective similar to that used in \citep{lee2023aligning}:

\begin{equation}
\mathbb{E}_{p(z)}\mathbb{E}_{p_{\text{pre}}(x_0|z)}[-r(x_0,z)\log p_\theta(x_0|z)].
\end{equation}

% \begin{lemma}
% \label{lemma_sup_reweight}
% Assume that 
% % , which is a reweighted version of the normal diffusion training using a pre-trained reward function
% \end{lemma}

% (another lemma here as 4.3, using similar approach in sup kl to show elbo for reward reweighting)

% \paragraph{KL regularization in a supervised manner.}

% First, we analyze the upper bound of the KL divergence between the pre-trained model and the current model during training.

% Let $p_{\text{pre}}(x_t|z)$ be the conditional probability of $x_t$ given $z$ from the pre-trained model. 
To compare with RL fine-tuning, we augment the supervised objective with a similar regularization: $\text{KL}(p_{\text{pre}}(x_0|z)\|p_\theta(x_0|z))$ in the supervised setting, which is equivalent to minimizing $\mathbb{E}_{p_{\text{pre}}(x_0|z)}[-\log{p_\theta(x_0|z)}]$ given any $z$.
Let $q(x_t)$ be the forward noising process used for training. Since the distribution of $x_0$ is generally not tractable, we use an approximate upper bound in the lemma below, which is similar to the DDPM training objective of~\citep{ho2020denoising}, but reweighted by the sum of reward and the regularization coefficient:

\begin{lemma}
\label{lemma_sup_kl}
Let $\gamma$ be the regularization weight. Assume $r(x_0,z) + \gamma > 0 $ for all $x_0, z$. 
% Define $q(x_0|z) := p_{\text{pre}}(x_0|z)$. 
% Assume that $p_{\text{pre}}(x_{1:T}|x_0) \approx q(x_{1:T}|x_0)$. 
Then:
\begin{equation}
\begin{aligned}
&\mathrel{\phantom{=}}\mathbb{E}_{p(z)}\mathbb{E}_{p_{\text{pre}}(x_0|z)}[-r(x_0,z)\log{p_\theta(x_0|z)}]+\gamma\mathbb{E}_{p(z)}\mathbb{E}_{p_{\text{pre}}(x_0|z)}[-\log{p_\theta(x_0|z)}] \\
& \leq \mathbb{E}_{p(z)}\mathbb{E}_{p_\text{pre}(x_0|z)}\left[(r(x_0,z)+\gamma)\mathbb{E}_{q(x_T|x_0,z)}[\text{\em KL}(q(x_T|x_0) \|p(x_T))] \right.\\
&\mathrel{\phantom{=}}+(r(x_0,z)+\gamma)\sum_{t>1} \mathbb{E}_{q(x_t|x_0,z)}[\text{\em KL}(q(x_{t-1}|x_t, x_0) \| p_\theta(x_{t-1}|x_t, z))] \\
&\left.\mathrel{\phantom{=}}+(r(x_0,z)+\gamma)\mathbb{E}_{q(x_1|x_0,z)}[-\log p_{\theta}(x_0|x_1, z)]\right].\\
% &\leq\mathbb{E}_{p(z)}\mathbb{E}_{p_{\text{pre}}(x_0|z)}[\mathbb{E}_{q(x_T|z, x_0)}[(r(x_0,z)+\gamma)KL(q(x_T|x_0) \\|p(x_T))]\\
% &\mathrel{\phantom{=}}+\sum_{t>1} \mathbb{E}_{q( x_t|x_0,z)}[(r(x_0,z)+\gamma)\frac{\|x_0 - f_{\theta}(x_t, t, z)\|^2}{2\sigma_t^2}]\\
% &\mathrel{\phantom{=}}-\mathbb{E}_{q(x_1|x_0,z)}[(r(x_0,z)+\gamma)\log p_{\theta}(x_0|z,x_1)]]\\
\end{aligned}
\end{equation}


% Let $f_{\theta}(x_t, t, z) := (x_t - \sqrt{1 -\alpha_t} \epsilon_{\theta}(x_t, t, z))/\sqrt{\alpha_t}$, $\sigma_t^2 := \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t}\beta_t$, we also have another weaker upper bound:

% \begin{equation}
% \begin{aligned}
% &\mathrel{\phantom{=}}\mathbb{E}_{p(z)}\mathbb{E}_{p_{\text{pre}}(x_0|z)}[-r(x_0,z)\log{p_\theta(x_0|z)}]+\gamma\mathbb{E}_{p(z)}\mathbb{E}_{p_{\text{pre}}(x_0|z)}[-\log{p_\theta(x_0|z)}]  \\
% &\leq\mathbb{E}_{p(z)}\mathbb{E}_{p_{\text{pre}}(x_0|z)}[\mathbb{E}_{q(x_T|z, x_0)}[(r(x_0,z)+\gamma)KL(q(x_T|x_0) \\|p(x_T))]\\
% &\mathrel{\phantom{=}}+\sum_{t>1} \mathbb{E}_{q( x_t|x_0,z)}[\frac{r(x_0,z)\|x_0 - f_{\text{pre}}(x_t, t,z)\|^2+\gamma\|f_{\text{pre}}(x_t, t,z)-f_{\theta}(x_t, t, z)\|^2}{2\sigma_t^2}]\\
% &\mathrel{\phantom{=}}-\mathbb{E}_{q(x_1|x_0,z)}[(r(x_0,z)+\gamma)\log p_{\theta}(x_0|z,x_1)]]\\
% \end{aligned}   
% \end{equation}


\end{lemma}
(See derivation in Appendix~\ref{proof_sup_kl}). 
% The assumption in Lemma~\ref{lemma_sup_kl} can be achieved when the pre-trained model is trained to convergence. 
This induces an supervised training objective with KL regularization:\footnote{$p_\theta(x_0|z, x_1)$ is modeled as a discrete decoder as in~\cite{ho2020denoising} and $p(x_T|z)$ is a fixed Gaussian;
% distribution, 
neither is trainable.}
\begin{equation}
\mathbb{E}_{p(z)}\mathbb{E}_{p_\text{pre}(x_0|z)}\left[(r(x_0,z)+\gamma)\sum_{t>1} \mathbb{E}_{q(x_t|x_0,z)}[\text{KL}(q(x_{t-1}|x_t, x_0) \| p_\theta(x_{t-1}|x_t, z))]\right],
\end{equation}
where we universally shift all rewards by some positive value $\gamma$, and treat it as the weight in supervised fine-tuning. The algorithm is described in Algorithm~\ref{alg:sup}. %\textcolor{red}{Do we need to provide more details like KL in eq10 is implemented as a simplified MSE loss? -- not imo, might be too detailed} 

% To minimize the bound, we need to add $\gamma$ to the reward function and use it as the weight for the MSE loss in diffusion training. 
Note that the supervised setting requires only a pre-trained diffusion model and no extra/new datasets as a fair comparison to online RL training.
% To minimize the last bound, besides training the diffusion model using the reweighted MSE loss, we can meanwhile punish the $L_2$ distance between the direction from pre-trained model and the current model.


% \paragraph{Objective function.}


% \begin{equation}
% \mathbb{E}_{p(z)}\mathbb{E}_{p_{\text{pre}}(x_0|z)}\left[- r(x,z)\log p_\theta(x_0|z)+\gamma \mathbb{E}_{q(x_0, x_t|z)}[\sum_{t>1} 
% \|\epsilon_{\text{pre}}(x_t, t, z) - \epsilon_{\theta}(x_t,t, z)\|^2]\right].
% \end{equation}

\begin{algorithm}[t]
  \caption{Supervised fine-tuning with human reward}

% \textbf{Require:} 
\textbf{Input}: Reward model $r$, pre-trained diffusion model $p_\text{pre}$, diffusion model $p_\theta$, regularization weight $\gamma$, batch size $n$, the number of training samples $M$

\begin{algorithmic}
\STATE Initialize $p_\theta = p_\text{pre}$
\STATE Collect $M$ samples from pre-trained model: $\mathcal{D} = \{(x_0, z)\sim p_\text{pre}(x_0|z)p(z) |\forall i \in \{1,...,M\}\}$
\WHILE{$\theta$ not converged}
 \STATE Obtain $n$ i.i.d. samples $\{x_0, z\}$ from training dataset $\mathcal{D}$
 %, by first sampling $z \sim p(z)$ and then $x_0 \sim p_\text{pre}(x_0|z)$  \textcolor{red}{nitpick: this is bit different from our implementation. We first generate dataset and then sample batch from fixed one. -- but it is the formal way to express that?} 
 \STATE Sample $x_t$ given $x_0$, $t \sim [1,T]$
 \STATE Take gradient step on $\nabla_\theta \big((r(x_0,z)+\gamma)\text{KL}(q(x_{t-1}|x_t, x_0) \| p_\theta(x_{t-1}|z, x_t))\big)$
%  \FOR{t = 0,...,$n_{\text{critic}}$}
% \STATE Obtain $m$ i.i.d. samples from $p^{\theta}_{x_{0:T}}$ and add to $\mathcal{B}$
% \STATE Obtain $m$ i.i.d. samples from $q_0$ 
% \STATE Update $\alpha$ and $\omega$ via maximizing Eq.~(\ref{eq: b and c})
% \ENDFOR
\ENDWHILE
\end{algorithmic}
\label{alg:sup}
\textbf{Output}: Fine-tuned diffusion model $p_\theta$
\end{algorithm}

\subsection{Contrasting Online RL Fine-tuning and Supervised Fine-tuning}
\label{sec:contrast}

We outline several key differences between online RL-based and supervised fine-tuning:

\begin{itemize} [leftmargin=7mm]
    \item \textbf{Online versus offline distribution.} We first contrast their objective. The online RL objective is to find a new image distribution that maximizes expected reward---this can have much different support than the pre-trained distribution. In supervised fine-tuning, the objective only encourages the model to ``imitate'' good examples from the supervised dataset, which always lies in the support of the pre-trained distribution.

    \item \textbf{Different KL regularization.} The methods also differ in their use of KL regularization. The supervised KL regularizer considers the upper bound of $\text{KL}(p_{\text{pre}}(x_0|z)\|p_\theta(x_0|z))$, while online KL regularizes the upper bound of $\text{KL}(p_\theta (x_0|z)) \| p_{\text{pre}}(x_0|z))$. More specifically, for online training, we evaluate conditional KL in each step using online samples, while for supervised training we evaluate conditional KL using supervised samples only.
    Moreover, online KL regularization can be seen as an extra reward function to encourage small divergence w.r.t. the pre-trained model for online optimization, while supervised KL induces an extra shift in the original reward for supervised training as shown in Lemma~\ref{lemma_sup_kl}. 
    % Due to the asymmetry of the KL divergence, online KL regularization constrains the relative entropy of $p_\theta$ with respect to $p_{\text{pre}}$, while supervised KL regularization punishes the relative entropy of $p_\text{pre}$ with respect to $p_{\theta}$.

    \item \textbf{Different evaluation of the reward model.} Online RL fine-tuning evaluates the reward model using its the updated distribution, while supervised fine-tuning evaluates the reward with the fixed, pre-train distribution.  As a consequence, our online RL optimization should derive greater benefit from the generalization ability of the reward model.
    
\end{itemize}

For these reasons, we expect online RL fine-tuning and supervised fine-tuning to generate rather different behaviors. Specifically, online fine-tuning should be better able to maximize the combined reward (human reward and implicit KL reward) than the supervised approach
% due to the ability of online optimization compared to supervised fine-tuning (which is
(similar to the difference between online learning and weighted behavior cloning in reinforcement learning).

==> sections/preliminary.tex <==
\section{Problem Setting} \label{sec:pre}

In this section, we describe our basic problem setting for text-to-image generation of diffusion models.

\paragraph{Diffusion models.}

We consider the use of \emph{denoising diffusion probabilistic models (DDPMs)}~\citep{ho2020denoising} for image generation. Let $q_0$ be the data distribution, i.e.,~$x_0 \sim q_0(x_0), \; x_0 \in \mathbb{R}^{n}$. A DDPM approximates $q_0$ with a parameterized model of the form $p_\theta(x_0)=\int p_\theta(x_{0:T})dx_{1:T}$. The 
% joint distribution $p_\theta(x_{0:T})$, dubbed the 
\emph{reverse process} is a Markov chain with the following dynamics:
%
\begin{equation}
\label{eq:reverse}
p_T(x_T) = \mathcal{N}(0, I), \qquad p_{\theta}(x_{t-1}|x_{t})=\mathcal{N}\big(\mu_\theta(x_{t},t), \Sigma_{t}\big).
\end{equation}
And we have $p_{\theta}({x_{0:T}} )= p_T(x_T)\prod_{t=1}^{T}p_{\theta}(x_{t-1}|x_t)$. A unique characteristic of DDPMs is the exploitation of an approximate posterior $q(x_{1:T}|x_0)$, known as the {\em forward} or {\em diffusion process}, which is itself a Markov chain that adds Gaussian noise to the data according to a variance schedule $\beta_1,\ldots,\beta_T$:
%
\begin{equation}
\label{eq:forward}
q(x_{1:T}|x_0) = \prod_{t=1}^T q(x_{t}|x_{t-1}), \qquad q(x_{t}|x_{t-1}) = \mathcal{N}(\sqrt{1-\beta_t}\;x_{t-1},\beta_tI). 
\end{equation}
%
Let $\alpha_{t} = 1-\beta_{t}$, $ \bar{\alpha}_{t} = \prod_{s=1}^{t}\alpha_{s}$, and 
$\tilde{\beta}_{t} = \frac{1 - \bar{\alpha}_{t-1}}{1 - \bar{\alpha}_{t}}\beta_{t}$. \citet{ho2020denoising} adopt the parameterization $\mu_\theta(x_t, t) = \frac{1}{\sqrt{\alpha_t}}\left(x_t - \frac{\beta_t}{\sqrt{1-\bar{\alpha}}_t}\epsilon_\theta(x_t,t)\right)$.

Training a DDPM is performed by optimizing a variational bound on the negative log-likelihood $\mathbb E[-\log p_\theta(x_0)]$, which is equivalent to optimizing: 
%
\begin{equation}
\label{eq:training}
\mathbb{E}_q\bigg[\sum_{t=1}^T\text{KL}\big(q(x_{t-1}|x_{t}, x_0)\| p_\theta(x_{t-1}|x_{t})\big)\bigg].
\end{equation}

% where $\tilde{\mu}_{t}(x_{t}, x_0) = \frac{\sqrt{\bar{\alpha}_t}\beta_{t-1}}{1-\bar{\alpha}_{t}}x_0 + \frac{\sqrt{\alpha_{t}}(1-\bar{\alpha}_{t-1})}{1-\bar{\alpha}_{t}}x_{t}$,

Note that the variance sequence $(\beta_t)_{t=1}^T \in (0,1)^T$ is chosen such that $\bar{\alpha}_T\approx 0$, and thus, $q(x_T|x_0) \approx \mathcal N(0,I)$. The covariance matrix $\Sigma_{t}$ in~\eqref{eq:reverse} is often set to either $\beta_{t}I$ or $\tilde{\beta}_{t}I$, which is not trainable.



% Here we consider denoising probabilistic diffusion models (DDPM)  as stochastic Markov chains with Gaussian noises~\citep{ho2020denoising}. 
% Consider data distribution $x_0 \sim q_0(x_0), x_0 \in \mathbb{R}^{n}$. 

% Define the forward noising process: for $t \in [0,..,T-1]$,
% \begin{equation}
%    q(x_{t+1}|x_{t}) := \mathcal{N}(\sqrt{1-\beta_t}x_{t}, \beta_tI), 
% \end{equation}
% where $x_1,.., x_T$ are variables of the same dimensionality as $x_0$, $\beta_{1:T}$ is the variance schedule. 

% We can compute the posterior as  a backward process:
% \begin{equation}
%     q(x_{t}|x_{t+1}, x_0) = \mathcal{N}(\tilde{\mu}_{t+1}(x_{t+1}, x_0), \tilde{\beta}_{t+1}I),
% \end{equation}
% where $\tilde{\mu}_{t+1}(x_{t+1}, x_0) = \frac{\sqrt{\bar{\alpha}_t}\beta_t}{1-\bar{\alpha}_{t+1}}x_0 + \frac{\sqrt{\alpha_{t+1}}(1-\bar{\alpha}_{t})}{1-\bar{\alpha}_{t+1}}x_{t+1}$, $\alpha_{t+1} = 1-\beta_{t+1}$, $ \bar{\alpha}_{t+1} = \prod_{s=1}^{t+1}\alpha_{s}$.

% We define a DDPM sampler parameterized by $\theta$, which generates data starting from some pure noise $x_T \sim p_T$:
% \begin{equation}
% \begin{split}
% &x_T \sim p_T = \mathcal{N}(0, I),\\
% &x_t \sim p_{\theta}(x_t|x_{t+1}),\\
% &p_{\theta}(x_t|x_{t+1}):=\mathcal{N}\big(\mu_{t+1}^\theta(x_{t+1}), \Sigma_{t+1}\big),\\
% \end{split}
% \end{equation}
% where $\Sigma_{t+1}$ is generally chosen as $\beta_{t+1}I$ or $\tilde{\beta}_{t+1}I$. 

% Define
% \begin{equation}
%    p_{\theta}({x_{0:T}} )= p_T(x_T)\prod_{t=0}^{T-1}p_{\theta}(x_t|x_{t+1}),
% \end{equation}
% and we have the marginal distribution $p_{\theta}(x_0) = \int p_{\theta}(x_{0:T}) d x_{1:T}$.


\paragraph{Text-to-image diffusion models.} 
Diffusion models are especially well-suited to \emph{conditional} data generation, as required by text-to-image models: one can plug in a classifier as guidance function~\citep{dhariwal2021diffusion}, or can directly train the diffusion model's  conditional distribution with classifier-free guidance \cite{ho2022classifier}.

Given text $z\sim p(z)$, let $q(x_0|z)$ be the conditional data distribution given the text prompt, which induces a joint distribution $p(x_0,z)$. During training, 
% they use 
the same noising process $q$ 
is used
regardless of input $z$, and both the unconditional denoising model $\epsilon_\theta(x_t,t)$ and a conditional denoising model $\epsilon_\theta(x_t,t, z)$ are learned. For data sampling, 
% they 
let $\bar{\epsilon}_\theta = w\epsilon_\theta(x_t,t, z) + (1-w) \epsilon_\theta(x_t,t)$, where $w\geq 1$ is a guidance scale. At test time, given a text prompt $z$, the model generates conditional data according to $p_\theta(x_0|z)$.

% \cb{Either start of end this section with a 1-2 sentence description of the TTI problem, e.g., relate text prompt and image output to the formal description of $q(x_0 | z)$.}


==> sections/relatedwork.tex <==
\section{Related Work} \label{sec:related_work}

% We being with a brief overview of related work.

\paragraph{Text-to-image diffusion models.}
Diffusion models~\cite{ho2020denoising,sohl2015deep,song2020improved} are a class of generative models that use an iterative denoising process to transform Gaussian noise into samples that follow a learned data distribution. These models have proven to be highly effective in a range of domains, including image generation~\cite{dhariwal2021diffusion}, audio generation~\cite{kong2020diffwave}, 3D synthesis~\cite{poole2022dreamfusion} and robotics~\cite{chi2023diffusion}. When combined with large-scale language encoders~\cite{clip,t5}, diffusion models have demonstrated impressive performance in text-to-image generation~\cite{dalle2,stablediffusion,imagen}. However, there are still many known weaknesses of existing text-to-image  models, such as compositionality and attribute binding \cite{feng2022training, liu2022compositional} or text rendering \cite{liu2022character}.
% However, despite these advances, current models are often lacking in certain~\cite{gokhale2022benchmarking,feng2022training,liu2022compositional,tifa}. For example, \citet{gokhale2022benchmarking} show that these models have a limited ability to produce multiple objects, or comprehend spatial relationships between objects. They also frequently encounter difficulties when generating fine-grained details, such as hands and faces~\cite{hps}.

% (cite stuff from SFT paper -- weaknesses in spatial relations, compositionality,  text generation) using RL from human feedback.
% \textcolor{red}{To-do: failure cases.}

\paragraph{Learning from human feedback.} Human assessments of (or preferences over) learned model outcomes have been used to guide learning on a variety of tasks, ranging from learning behaviors \cite{lee2021pebble} to language modeling \cite{bai2022training,ouyang2022training}. Recent work has also applied such methods to improve the alignment of text-to-image models.
% ceb: Redundant: this is all repeated below!
% typically by learning a \emph{reward model} from human assessments that is used to fine tune a pretrained text-to-image model. 
Human preferences are typically gathered at scale by asking annotators to compare generations, and a \emph{reward model} is trained (for example, by fine-tuning a vision-language model such as CLIP \cite{clip} or BLIP~\cite{blip}) to produce scalar rewards well-aligned with the human data \cite{imagereward, kirstain2023pick}. The reward model is used to improve text-to-image model quality by fine-tuning a pre-trained generative model \cite{lee2023aligning, wu2023better}. Unlike prior approaches, which typically focus on reward-filtered or reward-weighted supervised learning, we develop an online fine-tuning framework with an RL-based objective.  

\paragraph{RL fine-tuning of diffusion models.} \citet{fan2023optimizing} introduce a method to improve pre-trained diffusion models by integrating policy gradient and GAN training~\cite{goodfellow2020generative}. They use policy gradient with reward signals from the discriminator to update the diffusion model.
They demonstrate that the fine-tuned model can generate realistic samples with few steps with DDPM sampling~\cite{ho2020denoising} on relatively simple domains (e.g., CIFAR~\cite{cifar} and CelebA~\cite{celeba}. In this work, we explore RL fine-tuning especially for large-scale text-to-image models using human reward.
We also consider several design choices like adding KL regularization as the implicit reward, and compare RL fine-tuning to supervised fine-tuning.

% \textcolor{red}{[to-do] @ying: comparison with Sergey's work.}

% the sft paper and papers that cite the previous sft paper;
% \ow{
% \begin{itemize}
%     \item Maybe cite Stable Diffusion 2.0 release and describe the improvements they made.
%     \item All of the citation in the Aligning text-to-image models using human feedback seem relevant.
%     \item https://aaronlou.com/blog/2023/reflected-diffusion/
%     \item That one paper on human preferences for editing.
%     \item https://arxiv.org/pdf/2212.09611.pdf
%     \item (Maybe see if there's any analysis of RLHF in the language space analyzing when online training vs offline training is better.)
%     \item Maybe describe techniques commonly used for finetuning T2I models (e.g. LoRA). And maybe show papers which try other techniques (prompt tuning, just tuning attention, etc. I can find a list of these if you'd like.)
% \end{itemize}
% }
% \yd{describe imagereward}
